On the James and Hilton-Milnor Splittings, & the metastable EHP sequence

This note provides modern proofs of some classical results in algebraic topology, such as the James Splitting, the Hilton-Milnor Splitting, and the metastable EHP sequence. We prove fundamental splitting results \begin{equation*} \Sigma \Omega \Sigma X \simeq \Sigma X \vee (X\wedge \Sigma\Omega \Sigma X) \quad \text{and} \quad \Omega(X \vee Y) \simeq \Omega X\times \Omega Y\times \Omega \Sigma(\Omega X \wedge \Omega Y) \end{equation*} in the maximal generality of an $\infty$-category with finite limits and pushouts in which pushouts squares remain pushouts after basechange along an arbitrary morphism (i.e., Mather's Second Cube Lemma holds). For connected objects, these imply the classical James and Hilton-Milnor Splittings. Moreover, working in this generality shows that the James and Hilton-Milnor splittings hold in many new contexts, for example in: elementary $\infty$-topoi, profinite spaces, and motivic spaces over arbitrary base schemes. The splitting result in this last context extend Wickelgren and Williams' splitting result for motivic spaces over a perfect field. We also give two proofs of the metastable EHP sequence in the setting of $\infty$-topoi: the first is a new, non-computational proof that only utilizes basic connectedness estimates involving the James filtration and the Blakers-Massey Theorem, while the second reduces to the classical computational proof.

==> header.tex <==
%\usepackage{fullpage}
\usepackage[margin=1.175in]{geometry}	    
\pagestyle{plain}

\usepackage{amsmath}
\usepackage{amsthm}

%-------------------------------------------------------------------%
%  Typesetting                                                      %
%-------------------------------------------------------------------%

\usepackage[LGR,T1]{fontenc} % LGR allows for Greek text input
\usepackage[utf8]{inputenc} 
\RequirePackage[lcgreekalpha,upint]{stix2} % For older TeX distributions, use stix rather than stix2
\usepackage{inconsolata}
\newcommand{\mathup}[1]{\mathrm{#1}}
\newcommand{\mathbfup}[1]{\mathbf{#1}}
\newcommand{\el}{\ell}
\renewcommand{\in}{\smallin}
\newcommand{\textgreek}[1]{\begingroup\fontencoding{LGR}\selectfont#1\endgroup} % Creates an environment to input Greek text as unicode characters (while still using PDFLaTeX)


%-------------------------------------------------------------------%
%  Colors                                                           %
%-------------------------------------------------------------------%

\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

\definecolor{tulip}{RGB}{69, 9, 67}
\definecolor{love}{RGB}{128, 15, 37}
\definecolor{champ}{RGB}{249, 205, 173}
\definecolor{lobster}{RGB}{255, 64, 64}
\definecolor{dutch}{RGB}{22, 147, 165}
\definecolor{slate}{RGB}{42, 54, 59}

%-------------------------------------------------------------------%
%  Links                                                            %
%-------------------------------------------------------------------%

\usepackage{hyperref}
\hypersetup{
  colorlinks=true, %set true if you want colored links
  linktoc=all,     %set to all if you want both sections and subsections linked
  linkcolor=love,  %choose some color if you want links to stand out
  citecolor = love,
  urlcolor = slate,
  pdfencoding=unicode,
  % urlcolor=blue, % choose some color to set links to websites
  hypertexnames = true,
}
%%%%%%%%%%%%% for sanath
%\hypersetup{
%    colorlinks = true,
%    %allcolors = blue,
%    citecolor = [rgb]{0.00, 0.5, 0.00},
%}
%\usepackage{eucal}
%\usepackage{scalerel}
%  \newcommand{\similarrightarrow}{\mathrel{\ooalign{
%     $\to$\cr
%     \hidewidth\raise.3em\hbox{$\scaleobj{.5}{\sim}\mkern7mu$}\cr
%    }
%  }
%}

%-------------------------------------------------------------------%
%  Graphics                                                         %
%-------------------------------------------------------------------%

\usepackage{tikz}
\usepackage{tikz-cd}

\usetikzlibrary{matrix,arrows,arrows.meta,bending,calc,decorations,decorations.pathmorphing,shapes}

  \tikzset{
    RRight/.tip={Glyph[glyph math command=arrowkitHeadright]},
    double distance={0.135em},
    commutative diagrams/.cd, 
    arrow style=tikz, 
  }

  % tip end  -- 1
  % back end -- 0.00512821
  % line end -- 0.774359
  % visual back end -- 0.574359
  % visual tip end -- 1
  \pgfdeclarearrow{
      name = minionto,
      parameters = { \the\pgfarrowlength\the\pgfarrowwidth},
      setup code = {
          % The different end values:
          \pgfarrowssettipend{\pgfarrowlength}
          \pgfarrowssetbackend{0.00512821\pgfarrowlength}
          \pgfarrowssetlineend{0.774369\pgfarrowlength}
          \pgfarrowssetvisualbackend{0.574359\pgfarrowlength}
          \pgfarrowssetvisualtipend{\pgfarrowlength}
          % The hull
          \pgfarrowsupperhullpoint{0cm}{0.914141\pgfarrowwidth}
          \pgfarrowsupperhullpoint{0cm}{0.469697\pgfarrowwidth}
          \pgfarrowsupperhullpoint{0.107692\pgfarrowlength}{\pgfarrowwidth}
          \pgfarrowshullpoint{0.574359\pgfarrowlength}{0cm}
          \pgfarrowshullpoint{\pgfarrowlength}{0cm}
          % Saves: the length and width
          \pgfarrowssavethe\pgfarrowlength
          \pgfarrowssavethe\pgflinewidth
      },
      drawing code = {
          \pgfpathmoveto{\pgfpoint{0cm}{-0.914141\pgfarrowwidth}}
          \pgfpathlineto{\pgfpoint{0.574359\pgfarrowlength}{0cm}}
          \pgfpathlineto{\pgfpoint{0cm}{0.914141\pgfarrowwidth}}        
          \pgfpathlineto{\pgfpoint{0.107692\pgfarrowlength}{\pgfarrowwidth}}
          \pgfpathcurveto{\pgfpoint{0.528205\pgfarrowlength}{0.5\pgfarrowwidth}}
                         {\pgfpoint{0.548718\pgfarrowlength}{0.469697\pgfarrowwidth}}
                         {\pgfpoint{\pgfarrowlength}{0cm}}
          \pgfpathcurveto{\pgfpoint{0.528205\pgfarrowlength}{-0.5\pgfarrowwidth}}
                         {\pgfpoint{0.548718\pgfarrowlength}{-0.469697\pgfarrowwidth}}
                         {\pgfpoint{0.107692\pgfarrowlength}{-\pgfarrowwidth}}
          \pgfpathclose
          \pgfusepathqfill
      },
      defaults = {length=0.22em, width=0.19em}
  }

  \pgfarrowsdeclarereversed{miniontail}{miniontail}{minionto}{minionto}

  \pgfdeclarearrow{
      name = minionhook,
      parameters = { \the\pgflinewidth},
      setup code = {
          \pgfmathsetlength{\pgfarrowlength}{4.48\pgflinewidth}
          \pgfarrowssetlineend{\pgflinewidth}
          \pgfarrowssettipend{\pgfarrowlength}
          % The hull
          \pgfarrowsupperhullpoint{0cm}{0.914141\pgflinewidth}
          \pgfarrowsupperhullpoint{0cm}{0.469697\pgflinewidth}
          \pgfarrowsupperhullpoint{0.107692\pgfarrowlength}{\pgflinewidth}
          \pgfarrowshullpoint{0.574359\pgfarrowlength}{0cm}
          \pgfarrowshullpoint{\pgfarrowlength}{0cm}
          % Saves: the length and width
          \pgfarrowssavethe\pgflinewidth
          \pgfarrowssavethe\pgfarrowlength
      },
      drawing code = {
          \pgfpathmoveto{\pgfpoint{0.25\pgfarrowlength}{-3.84\pgflinewidth}}
          \pgfpathlineto{\pgfpoint{0.25\pgfarrowlength}{-2.86\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.73660714\pgfarrowlength}{-2.86\pgflinewidth}}
                         {\pgfpoint{0.73660714\pgfarrowlength}{-1.9\pgflinewidth}}
                         {\pgfpoint{0.73660714\pgfarrowlength}{-1.6\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.73660714\pgfarrowlength}{-0.54\pgflinewidth}}
                         {\pgfpoint{0.35267857\pgfarrowlength}{-0.45\pgflinewidth}}
                         {\pgfpoint{0.0\pgfarrowlength}{-0.51\pgflinewidth}}
          \pgfpathlineto{\pgfpoint{0.0\pgfarrowlength}{0.5\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.97767857\pgfarrowlength}{0.7\pgflinewidth}}
                         {\pgfpoint{0.99107143\pgfarrowlength}{-1.2\pgflinewidth}}
                         {\pgfpoint{1.0\pgfarrowlength}{-1.6\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.95982143\pgfarrowlength}{-3.86\pgflinewidth}}
                         {\pgfpoint{0.39732143\pgfarrowlength}{-3.86\pgflinewidth}}
                         {\pgfpoint{0.25\pgfarrowlength}{-3.86\pgflinewidth}}
          \pgfpathclose
          \pgfusepathqfill
      },
      defaults = {length=0.22em, width=0.19em}
  }

  \pgfdeclarearrow{
      name = minionhook',
      parameters = { \the\pgflinewidth},
      setup code = {
          \pgfmathsetlength{\pgfarrowlength}{4.48\pgflinewidth}
          \pgfarrowssetlineend{\pgflinewidth}
          \pgfarrowssettipend{\pgfarrowlength}
          % The hull
          \pgfarrowsupperhullpoint{0cm}{0.914141\pgflinewidth}
          \pgfarrowsupperhullpoint{0cm}{0.469697\pgflinewidth}
          \pgfarrowsupperhullpoint{0.107692\pgfarrowlength}{\pgflinewidth}
          \pgfarrowshullpoint{0.574359\pgfarrowlength}{0cm}
          \pgfarrowshullpoint{\pgfarrowlength}{0cm}
          % Saves: the length and width
          \pgfarrowssavethe\pgflinewidth
          \pgfarrowssavethe\pgfarrowlength
      },
      drawing code = {
          \pgfpathmoveto{\pgfpoint{0.25\pgfarrowlength}{3.84\pgflinewidth}}
          \pgfpathlineto{\pgfpoint{0.25\pgfarrowlength}{2.86\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.73660714\pgfarrowlength}{2.86\pgflinewidth}}
                         {\pgfpoint{0.73660714\pgfarrowlength}{1.9\pgflinewidth}}
                         {\pgfpoint{0.73660714\pgfarrowlength}{1.6\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.73660714\pgfarrowlength}{0.54\pgflinewidth}}
                         {\pgfpoint{0.35267857\pgfarrowlength}{0.45\pgflinewidth}}
                         {\pgfpoint{0.0\pgfarrowlength}{0.51\pgflinewidth}}
          \pgfpathlineto{\pgfpoint{0.0\pgfarrowlength}{-0.5\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.97767857\pgfarrowlength}{-0.7\pgflinewidth}}
                         {\pgfpoint{0.99107143\pgfarrowlength}{1.2\pgflinewidth}}
                         {\pgfpoint{1.0\pgfarrowlength}{1.6\pgflinewidth}}
          \pgfpathcurveto{\pgfpoint{0.95982143\pgfarrowlength}{3.86\pgflinewidth}}
                         {\pgfpoint{0.39732143\pgfarrowlength}{3.86\pgflinewidth}}
                         {\pgfpoint{0.25\pgfarrowlength}{3.86\pgflinewidth}}
          \pgfpathclose
          \pgfusepathqfill
      },
      defaults = {length=0.22em, width=0.19em}
  }

  \tikzset{
    >/.tip={minionto},
    >->/.style = {miniontail-minionto},
    <-</.style = {minionto-miniontail},
    <->/.style = {minionto-miniontail},
    hooked/.style = {minionhook-minionto},
    hooked'/.style = {minionhook'-minionto},
  }

  \tikzset{
  RRight/.tip={Glyph[glyph math command=arrowkitHeadright]},
}

\pgfdeclaredecoration{single line}{initial}{\state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfpathmoveto{\pgfpointorigin}}\state{final}{\pgfpathlineto{\pgfpointorigin}}}

% Sets global tikzcd settings
\tikzcdset{  crossing over/.style={
    /tikz/preaction={
      /tikz/draw,
      /tikz/color=\pgfkeysvalueof{/tikz/commutative diagrams/background color},
      /tikz/arrows=-,
      /tikz/line width=\pgfkeysvalueof{/tikz/commutative
      diagrams/crossing over clearance}}}}

%-------------------------------------------------------------------%
%  References                                                       %
%-------------------------------------------------------------------%


% Uses biblatex pacage for citations and sets basic global styling
%-------------------------------------------------------------------%

\usepackage[style=ieee,citestyle=numeric,backend=biber,bibencoding=utf8,sorting=nyt,url=false]{biblatex} % url=false removes '[Online] Available: _repetition of DOI_'
\AtEveryBibitem{\clearfield{issn}} % Removes ISSN (retains ISBN)
\AtEveryCitekey{\clearfield{issn}}
\AtBeginBibliography{\small} % Sets references font size
\renewcommand*{\bibnamedash}{\underline{\hspace{3em}}\kern 0.1em} % Uses an underline when an author has multiple publications (in line with the AMS style)
\renewcommand{\multicitedelim}{\addsemicolon\space} % Uses a semicolon delimeter for multiple citations
\DeclareFieldFormat{postnote}{#1} % Removes the "p." when just a number is referenced
\DeclareFieldFormat[article,inbook,incollection,inproceedings,patent,thesis,unpublished]
  {title}{\textit{#1\isdot}}     % Uniformly italicizes title of all works
\DeclareFieldFormat{journaltitle}{#1}  % Makes Journal title in normal text
\DeclareFieldFormat[book,inbook,incollection,inproceedings]{series}{#1} % Takes away the "ser." in front of Series Title that is part of the ieee styling

% Definition of various links to make it easy to hyperlink to the Stacks project and the books of Jacob
%-------------------------------------------------------------------%

\newcommand{\stackslink}[1]{\href{http://stacks.math.columbia.edu/tag/#1}{#1}} % For use with multiple references

\newcommand{\kerodonlink}[1]{\href{http://kerodon.net/tag/#1}{#1}} % For use with multiple references

% Part Links
\newcommand{\SAGpartlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#part.#1}{#1}}

% Chapter Links
\newcommand{\HTTchlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#chapter.#1}{#1}}
\newcommand{\HAchlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#chapter.#1}{#1}}
\newcommand{\SAGchlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#chapter.#1}{#1}}

% Appendix Links
\newcommand{\HTTapplink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#appendix.#1}{#1}}
\newcommand{\HAapplink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#appendix.#1}{#1}}
\newcommand{\SAGapplink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#appendix.#1}{#1}}

% Section Links
\newcommand{\HTTseclink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#section.#1}{#1}}
\newcommand{\HAseclink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#section.#1}{#1}}
\newcommand{\SAGseclink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#section.#1}{#1}}

% Subsection Links
\newcommand{\HTTsubseclink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#subsection.#1}{#1}}
\newcommand{\HAsubseclink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#subsection.#1}{#1}}
\newcommand{\SAGsubseclink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#subsection.#1}{#1}}

% Theorem/Lemma/Definition/etc. Links
\newcommand{\HTTthmlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#theorem.#1}{#1}}
\newcommand{\HAthmlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#theorem.#1}{#1}}
\newcommand{\HAappthmlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#atheorem.#1}{#1}} % Appendix theorems are numbered differently
\newcommand{\SAGthmlink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#theorem.#1}{#1}}

% Page Links
\newcommand{\HTTpagelink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#page.#1}{#1}}
\newcommand{\HApagelink}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#page.#1}{#1}}
\newcommand{\SAGpagelink}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#page.#1}{#1}}

% Definition of various references to make it easy to hyperlink to the Stacks project and the books of Jacob
%-------------------------------------------------------------------%

\newcommand{\stackstag}[1]{\href{http://stacks.math.columbia.edu/tag/#1}{Tag #1}} %for single reference use

\newcommand{\kerodontag}[1]{\href{http://kerodon.net/tag/#1}{Tag #1}} %for single reference use

% Part Reference
\newcommand{\SAGpart}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#part.#1}{Part #1}}

% Chapter Reference
\newcommand{\HTTch}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#chapter.#1}{Chapter #1}}
\newcommand{\HAch}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#chapter.#1}{Chapter #1}}
\newcommand{\SAGch}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#chapter.#1}{Chapter #1}}

% Appendix Reference
\newcommand{\HTTapp}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#appendix.#1}{Appendix #1}}
\newcommand{\HAapp}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#appendix.#1}{Appendix #1}}
\newcommand{\SAGapp}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#appendix.#1}{Appendix #1}}

% Section Reference
\newcommand{\HTTsec}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#section.#1}{\S #1}}
\newcommand{\HAsec}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#section.#1}{\S #1}}
\newcommand{\SAGsec}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#section.#1}{\S #1}}

% Subsection Reference
\newcommand{\HTTsubsec}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#subsection.#1}{\S #1}}
\newcommand{\HAsubsec}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#subsection.#1}{\S #1}}
\newcommand{\SAGsubsec}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#subsection.#1}{\S #1}}

% Theorem/Lemma/Definition/etc. Reference
\newcommand{\HTTthm}[2]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#theorem.#2}{#1 #2}}
\newcommand{\HAthm}[2]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#theorem.#2}{#1 #2}}
\newcommand{\HAappthm}[2]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#atheorem.#2}{#1 #2}} % Appendix theorems are numbered differently
\newcommand{\SAGthm}[2]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#theorem.#2}{#1 #2}}

% Page Reference
\newcommand{\HTTpage}[1]{\href{http://www.math.ias.edu/~lurie/papers/HTT.pdf\#page.#1}{p. #1}}
\newcommand{\HApage}[1]{\href{http://www.math.ias.edu/~lurie/papers/HA.pdf\#page.#1}{p. #1}}
\newcommand{\SAGpage}[1]{\href{http://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf\#page.#1}{p. #1}}

% Quick Citation command for citing a single theorem, lemma, etc. 
%-------------------------------------------------------------------%

% Use: for stacks \stacks{Tag Number}, for HTT/HA/SAG, e.g., \HTT{Environment name}{Number}

\newcommand{\stacks}[1]{\cite[\stackstag{#1}]{stacksproject}}
\newcommand{\kerodon}[1]{\cite[\kerodontag{#1}]{Kerodon}}
\newcommand{\HTT}[2]{\cite[\HTTthm{#1}{#2}]{HTT}}
\newcommand{\HA}[2]{\cite[\HAthm{#1}{#2}]{HA}}
\newcommand{\HAa}[2]{\cite[\HAappthm{#1}{#2}]{HA}} % For theorems in the appendix of HA because the numbering is different
\newcommand{\SAG}[2]{\cite[\SAGthm{#1}{#2}]{SAG}}

%-------------------------------------------------------------------%
% cleverref package 
%-------------------------------------------------------------------%

\usepackage[noabbrev,nameinlink,capitalize]{cleveref} % Uses the cleveref package for convenient within-document referencing. The placement of this package IS IMPORTANT. (It may not work if it is placed in a different order with respect to other packages.)

% The commands below specify how the cleveref package names different environments when they are cited. There are two options, "\cref" and "\Cref". I've used \cref for abbreviated forms and \Cref for long forms. We can cange any and all of these; I just used put some things that seemed standard.

% Has cref parenthesize "nul" references
\crefformat{nul}{(#2#1#3)}
\Crefformat{nul}{(#2#1#3)}

\crefname{section}{\S\!}{\S\S\!}
\crefname{subsection}{\S\!}{\S\S\!}
\crefname{axioms}{Axiom}{Axioms}
\crefname{exercise}{Exercise}{Exercises}
\crefname{exercisenum}{Exercise}{Exercises}
\crefname{construction}{Construction}{Constructions}
\crefname{problem}{Problem}{Problems}
\crefname{theorem}{Theorem}{Theorems}
\crefname{definition}{Definition}{Definitions}
\crefname{prop}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{example}{Example}{Examples}
\crefname{examplealph}{Example}{Examples}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{nonexample}{Nonexample}{Nonexamples}
\crefname{recollection}{Recollection}{Recollections}
\Crefname{recollection}{Recollection}{Recollections}
\Crefname{nonexample}{Nonexample}{Nonexamples}
\Crefname{corollary}{Corollary}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}
\Crefname{axioms}{Axiom}{Axioms}
\Crefname{exercise}{Exercise}{Exercises}
\Crefname{exercisenum}{Exercise}{Exercises}
\Crefname{construction}{Construction}{Constructions}
\Crefname{problem}{Problem}{Problems}
\Crefname{theorem}{Theorem}{Theorems}
\Crefname{definition}{Definition}{Definitions}
\Crefname{prop}{Proposition}{Propositions}
\Crefname{lemma}{Lemma}{Lemmas}
\Crefname{example}{Example}{Examples}
\Crefname{examplealph}{Example}{Examples}
\Crefname{section}{Section}{Sections}
\Crefname{subsection}{Subsection}{Subsections}


\usepackage{mathtools}

%\usepackage{txfonts} % Thanks to Eric for showing me that this font exists.

%\usepackage{libertine}
%\usepackage{libertinust1math}
%\usepackage[T1]{fontenc}

%\usepackage[urw-garamond]{mathdesign}

%\usepackage[disable]{todonotes}
\usepackage{todonotes}
\usepackage{multirow}
\usepackage{longtable}


% \usepackage{amsfonts}
\let\centerdot\undefined % here - PS
\let\circledS\undefined % here - PS
% \usepackage{amssymb}
\usepackage{float}
\usepackage{comment}
% \usepackage{amscd}
% \usepackage{amsxtra}
% \usepackage{epsfig}
%\usepackage{MnSymbol}

\usepackage{listings}
\usepackage{color}

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=Java,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}

\usepackage{color}
% \usepackage[all]{xy}
\usepackage{verbatim}

% \usepackage{mathrsfs}

\usepackage{graphicx}
% \usepackage{tikz-cd}

%\xyoption{all}
\usepackage{url}
\usepackage{verbatim}
%\urlstyle{rm}

\usepackage{xy}
%\input xy
\xyoption{all}
%%\setcounter{tocdepth}{1}
\newcommand{\xar}[1]{\xrightarrow{{#1}}}

% \usepackage{amsthm}

%\usepackage{tikz}
%\usepackage{cleveref/cleveref}

\usepackage{caption} 
\captionsetup[table]{skip=-10pt}

\makeatletter
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima
      \ifcase #1
       \or\or \hskip 1em \or \hskip 2em \else \hskip 3em \fi%
      #6\nobreak\relax
    \hfill\hbox to\@pnumwidth{\@tocpagenum{#7}}\par% <---- \dotfill -> \hfill
    \nobreak
    \endgroup
  \fi}
\makeatother

\DeclareMathOperator{\Fun}{Fun}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Alt}{Alt}
\DeclareMathOperator{\spec}{Spec}
\DeclareMathOperator{\spf}{Spf}
\DeclareMathOperator{\spa}{Spa}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\supp}{Supp}
\DeclareMathOperator{\RHom}{RHom}
\DeclareMathOperator{\red}{red}
\DeclareMathOperator{\picsp}{\mathfrak{pic}}
\DeclareMathOperator{\coker}{coker}
\newcommand{\cofib}{\ensuremath{\textup{cofib}}}
\newcommand{\fib}{\ensuremath{\textup{fib}}}
\DeclareMathOperator{\perf}{perf}
\DeclareMathOperator{\Frob}{Frob}
\DeclareMathOperator{\QCoh}{\operatorname{QCoh}}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\pic}{Pic}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\hocolim}{hocolim}
\DeclareMathOperator{\holim}{holim}
\DeclareMathOperator{\Tot}{Tot}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\proj}{Proj}
\DeclareMathOperator{\sub}{Sub}

\renewcommand{\hom}{\operatorname{Hom}}

\numberwithin{equation}{section}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{sublemma}{Sublemma}
\newtheorem{corollary}[equation]{Corollary}
\newcommand{\bR}{{\mathbf R}}
\newcommand{\sO}{\mathcal{O}}
\newtheorem{fact}[equation]{Fact}
\newtheorem{qthm}[equation]{Quasi-Theorem}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem*{thm}{Theorem}
\newtheorem*{thmno}{Theorem}
\newtheorem*{propo}{Proposition}
\newtheorem{prop}[equation]{Proposition}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem*{conjectureno}{Conjecture}

\newtheorem{abc}{abc}
\newtheorem{letterprop}[abc]{Proposition}
\renewcommand*{\theabc}{\Alph{abc}}

\theoremstyle{definition}

\newtheorem{question}[equation]{Question}
\newtheorem{assumption}[equation]{Assumption}
\newtheorem{definition}[equation]{Definition}
\newtheorem{convention}[equation]{Convention}
\newtheorem{warning}[equation]{Warning}
\newtheorem{example}[equation]{Example}
\newtheorem{problem}[equation]{Problem}
\newtheorem{construction}[equation]{Construction}
\newtheorem{remark}[equation]{Remark}
\newtheorem{notation}[equation]{Notation}
\newtheorem{terminology}[equation]{Terminology}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{recollection}[equation]{Recollection}
\newtheorem{slogan}{Slogan}
\newtheorem*{acknowledgements}{Acknowledgements}

\renewcommand{\AA}{\mathbf{A}}
\newcommand{\FF}{\mathbf{F}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\QQ}{\mathbf{Q}}
\newcommand{\cc}{\mathbf{C}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cd}{\mathcal{D}}
\newcommand{\RR}{\mathbf{R}}
\newcommand{\Deltab}{\mathbf{\Delta}}
\newcommand{\Set}{\operatorname{Set}}
\newcommand{\Lp}{L_{K(p-1)}}
% \newcommand{\Lt}{L_{T(n)}}
\newcommand{\Lk}{L_{K(n)}}
\newcommand{\Ln}{L_n}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\sph}{\mathbf{S}^0}

\newcommand{\Aff}[1]{{\operatorname{Aff}^{\operatorname{et}}_{/#1}}}

\newcommand{\M}{{M}}
%\newcommand{\M}{\mathcal{M}}
\newcommand{\Mfg}{\M_{FG}}
\newcommand{\Mcub}{\M_\operatorname{cub}}
\newcommand{\Mell}{\M_\operatorname{ell}}
\newcommand{\sm}{\operatorname{sm}}

\newcommand{\Aoo}{{A_\infty}}
\newcommand{\ff}{\mathcal{F}}
\newcommand{\co}{\mathcal{O}}
\newcommand{\ce}{\mathcal{E}}
\newcommand{\TT}{\mathbf{T}}
\newcommand{\PP}{\mathbf{P}}
\renewcommand{\SS}{\mathbf{S}}
\newcommand{\GG}{\mathbb{G}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\map}{\operatorname{Map}}
\newcommand{\LMod}{\operatorname{LMod}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\cL}{\mathcal{L}}

%\newcommand{\CP}{\mathbf{CP}}
%\newcommand{\RP}{\mathbf{RP}}

\newcommand{\CC}{\mathcal{C}}
\newcommand{\HP}{\mathbf{H}P}
\newcommand{\CP}{\mathbf{C}P}
\newcommand{\RP}{\mathbf{R}P}


\newcommand{\Map}{\operatorname{Map}}

\newcommand{\dY}{\mathcal{Y}}
\newcommand{\dZ}{\mathcal{Z}}
\newcommand{\dV}{\mathcal{V}}
\newcommand{\dU}{\mathcal{U}}
\newcommand{\dX}{\mathcal{X}}

%\newcommand{\dY}{\mathfrak{Y}}
%\newcommand{\dZ}{\mathfrak{Z}}
%\newcommand{\dV}{\mathfrak{V}}
%\newcommand{\dU}{\mathfrak{U}}
%\newcommand{\dX}{\mathfrak{X}}

\newcommand{\frakm}{\mathfrak{m}}
\newcommand{\LTone}{L_{T(1)}}
\newcommand{\LTtwo}{L_{T(2)}}
\newcommand{\Lone}{L_{K(1)}}
\newcommand{\Ltwo}{L_{K(2)}}
\newcommand{\comm}{\operatorname{Comm}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\cg}{\mathcal{G}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\A}{\widehat{A}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\T}{\widetilde{T}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\Ab}{\operatorname{Ab}}
\newcommand{\calg}{\operatorname{CAlg}}
\newcommand{\der}{\operatorname{der}}
\newcommand{\Alg}{\operatorname{Alg}}
\renewcommand{\P}{{P}}
\newcommand{\Sq}{\operatorname{Sq}}
\newcommand{\nuca}{\operatorname{NUCA}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Q}{\underline{Q}}
\newcommand{\NN}{\mathbf{N}}
\newcommand{\TM}{T\mathcal{M}}
\newcommand{\e}{E_{12}}
\newcommand{\f}{F}
\newcommand{\m}{\mathfrak{m}}
\newcommand{\R}{\mathcal{R}}

\newcommand{\Eoo}{{\mathbf{E}_\infty}}
\newcommand{\EOo}{{\mathbf{E}_\infty}}

%\newcommand{\Eoo}{{E_\infty}}
%\newcommand{\EOo}{{E_\infty}}

\newcommand{\set}{\operatorname{Set}}
\newcommand{\CAlg}{\operatorname{CAlg}}
\newcommand{\Nm}{\operatorname{Nm}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cf}{\mathcal{F}}
\newcommand{\DD}{\mathbf{D}}
\newcommand{\dMfg}{\mathfrak{M}_\textbf{fg}}
\newcommand{\LT}{\operatorname{LT}}
\newcommand{\univ}{\operatorname{univ}}
\newcommand{\dR}{\operatorname{dR}}
\newcommand{\cris}{\operatorname{cris}}

\newcommand{\Def}{\operatorname{Def}}
\newcommand{\isog}{\operatorname{isog}}
\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Lie}{\operatorname{Lie}}
\newcommand{\Exc}{\operatorname{Exc}}
\newcommand{\fin}{\operatorname{fin}}
\newcommand{\Shv}{{\operatorname{Shv}}}
\newcommand{\Sm}{{\operatorname{Sm}}}
\newcommand{\Top}{{\operatorname{Top}}}
\newcommand{\ev}{\operatorname{ev}}
\newcommand{\Homo}{\operatorname{Homog}}
\newcommand{\Nilp}{\operatorname{Nilp}}
\newcommand{\cP}{\mathcal{P}} % presheaves
\newcommand{\cH}{\mathcal{H}}
\newcommand{\Sh}{\operatorname{Sh}}
\newcommand{\TAF}{\operatorname{TAF}}
\newcommand{\cN}{\mathcal{N}}

\newcommand{\Lonen}{L_{K(1)\vee\cdots\vee K(n)}}

\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\coord}{\operatorname{coord}}
\newcommand{\Perf}{\operatorname{Perf}}

\newcommand{\D}{\operatorname{D}}
\newcommand{\DM}{\operatorname{DM}}
\newcommand{\E}[1]{\mathbf{E}_{{#1}}}
\newcommand{\mmod}{/\!\!/}
\newcommand{\prim}{\operatorname{Prim}}

\renewcommand{\sp}{\mathbin{\rotatebox[origin=c]{-90}{Y}}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Stab}{\operatorname{Stab}}
\renewcommand{\theenumi}{\alph{enumi}}

%\newcommand{\bgl}{{bgl}}
%\newcommand{\gl}{{gl}}
%\newcommand{\SL}{{SL}}
%\newcommand{\GL}{{GL}}
%\newcommand{\MUP}{{MUP}}
%\newcommand{\MU}{{MU}}
%\newcommand{\BU}{{BU}}
%\renewcommand{\O}{{O}}
%\newcommand{\SO}{{SO}}
%\newcommand{\BO}{{BO}}
%\newcommand{\KU}{{KU}}
%\newcommand{\KO}{{KO}}
%\newcommand{\ku}{{ku}}
%\newcommand{\ko}{{ko}}
%\newcommand{\bu}{{ku}}
%\newcommand{\bo}{{ko}}
%\newcommand{\EO}{{EO}}
%\newcommand{\tmf}{{tmf}}
%\newcommand{\Tmf}{{Tmf}}
%\newcommand{\TMF}{{TMF}}
%\newcommand{\BP}[1]{{BP}\langle{#1}\rangle}
%\newcommand{\SU}{{SU}}
%\newcommand{\BPP}{{BP}}
%\newcommand{\BSpin}{{BSpin}}
%\newcommand{\MSpin}{{MSpin}}
%\newcommand{\MString}{{MString}}
%\newcommand{\BString}{{BString}}
%\renewcommand{\H}{{H}}

\newcommand{\bgl}{\operatorname{bgl}}
\newcommand{\gl}{\operatorname{gl}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\MUP}{\operatorname{MUP}}
\newcommand{\MU}{\operatorname{MU}}
\newcommand{\BU}{\operatorname{BU}}
% \renewcommand{\O}{\operatorname{O}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\BO}{\operatorname{BO}}
\newcommand{\KU}{\operatorname{KU}}
\newcommand{\KO}{\operatorname{KO}}
\newcommand{\ku}{\operatorname{ku}}
\newcommand{\ko}{\operatorname{ko}}
\newcommand{\bu}{\operatorname{ku}}
\newcommand{\bo}{\operatorname{ko}}
\newcommand{\EO}{\operatorname{EO}}
\newcommand{\tmf}{\operatorname{tmf}}
\newcommand{\Tmf}{\operatorname{Tmf}}
\newcommand{\TMF}{\operatorname{TMF}}
\newcommand{\BP}[1]{\operatorname{BP}\langle{#1}\rangle}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\BPP}{\operatorname{BP}}

%\renewcommand{\H}{{H}}
\renewcommand{\H}{\operatorname{H}}

% don't change these...
\newcommand{\BSpin}{\operatorname{BSpin}}
\newcommand{\MSO}{\operatorname{MSO}}
\newcommand{\MSpin}{\operatorname{MSpin}}
\newcommand{\MString}{\operatorname{MString}}
\newcommand{\BString}{\operatorname{BString}}
\newcommand{\bso}{\operatorname{bso}}
\newcommand{\bspin}{\operatorname{bspin}}
\newcommand{\bstring}{\operatorname{bstring}}


\newcommand{\cross}{\operatorname{cr}}
\newcommand{\Conf}{\operatorname{Conf}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\THH}{\operatorname{THH}}
\newcommand{\fp}{\operatorname{fp}}
\newcommand{\la}[1]{\langle #1 \rangle}
\newcommand{\Free}{\operatorname{Free}}

\newcommand{\fr}[1]{\mathcal{#1}}
%\newcommand{\fr}[1]{\mathfrak{#1}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\CE}{\operatorname{CE}}
\newcommand{\KI}{\operatorname{KI}}

